Heterogeneity-Aware Cluster Scheduling Policies for Deep Learning Workloads

Specialized accelerators such as GPUs, TPUs, FPGAs, and custom ASICs have been increasingly deployed to train deep learning models. These accelerators exhibit heterogeneous performance behavior across model architectures. Existing schedulers for clusters of accelerators, which are used to arbitrate these expensive training resources across many users, have shown how to optimize for various multi-job, multi-user objectives, like fairness and makespan. Unfortunately, existing schedulers largely do not consider performance heterogeneity. In this paper, we propose Gavel, a heterogeneity-aware scheduler that systematically generalizes a wide range of existing scheduling policies. Gavel expresses these policies as optimization problems, making it easy to optimize for objectives in a heterogeneity-aware way, while also being cognizant of performance optimizations like space sharing. Gavel then uses a round-based scheduling mechanism to ensure jobs receive their ideal allocation given the target scheduling policy. Gavel's heterogeneity-aware policies allow a heterogeneous cluster to sustain higher input load, and improve end objectives such as average job completion time and makespan by up to 3.5x compared to heterogeneity-agnostic policies.

==> acknowledgements.tex <==
\section{Acknowledgements}

We thank Firas Abuzaid, Trevor Gale, Kshiteej Mahajan, Shoumik Palkar,
Deepti Raghavan, Daniel Kang, Pratiksha Thaker, and Jayashree Mohan for their
invaluable feedback that made this work better.

==> mechanism_figures.tex <==
\begin{figure*}
    \begin{subfigure}{0.68\columnwidth}
        \includegraphics[width=1.0\columnwidth]{figures/allocation_equal.pdf}
        \caption{
        \small Equal GPU-time allocation $X^\text{isolated}$.}
    \end{subfigure} \hfill
    \begin{subfigure}{0.68\columnwidth}
        \includegraphics[width=1.0\columnwidth]{figures/allocation_unequal.pdf}
        \caption{
        \small Heterogeneity-aware allocation $X^{\text{het.}}$.}
    \end{subfigure} \hfill
    \begin{subfigure}{0.68\columnwidth}
        \includegraphics[width=1.0\columnwidth]{figures/allocation_unequal_packing.pdf}
        \caption{
        \small Packing-aware allocation $X^{\text{het.+packing}}$.}
    \end{subfigure}
    \caption{
        \label{fig:scheduling_mechanism}
        Scheduling mechanism in action for various allocations. Space sharing is shown
        with vertically split boxes. Each round is denoted by a box. Numbers in boxes
        represent Job IDs. Heterogeneous-aware and packing-aware policies help reduce
        job completion times. Job completion times are computed under the assumption that each job has a duration of 100 rounds on a K80 GPU.
    }
    \vspace{-5mm}
\end{figure*}

